Perfusion Imaging: A Data Assimilation Approach

Perfusion imaging (PI) is clinically used to assess strokes and brain tumors. Commonly used PI approaches based on magnetic resonance imaging (MRI) or computed tomography (CT) measure the effect of a contrast agent moving through blood vessels and into tissue. Contrast-agent free approaches, for example, based on intravoxel incoherent motion, also exist, but are so far not routinely used clinically. These methods rely on estimating on the arterial input function (AIF) to approximately model tissue perfusion, neglecting spatial dependencies, and reliably estimating the AIF is also non-trivial, leading to difficulties with standardizing perfusion measures. In this work we therefore propose a data-assimilation approach (PIANO) which estimates the velocity and diffusion fields of an advection-diffusion model that best explains the contrast dynamics. PIANO accounts for spatial dependencies and neither requires estimating the AIF nor relies on a particular contrast agent bolus shape. Specifically, we propose a convenient parameterization of the estimation problem, a numerical estimation approach, and extensively evaluate PIANO. We demonstrate that PIANO can successfully resolve velocity and diffusion field ambiguities and results in sensitive measures for the assessment of stroke, comparing favorably to conventional measures of perfusion.

==> sub/bib.tex <==
\bibliographystyle{IEEEtran}
 \bibliography{sub/references}

==> sub/exp_results/box_plots_tmi.tex <==
\begin{figure}[t]
	\noindent\resizebox{\textwidth}{!}{
	\begin{tikzpicture}
	% Lesion
	\node at (0, 2.25) {\includegraphics[width=4cm]{fig/box_plots/rMean_rSTD.eps}};
	
	%\node at (4.2, 2.25) {\includegraphics[width=4.25cm]{fig/box_plots/t.eps}};
	\node at (0, -0.75) {\includegraphics[width=4cm]{fig/box_plots/t.eps}};
	\draw (-1.46 , -2.2) node[draw,scale=0.2,circle,line width=0.075mm]{}; 
	\draw (-1.31 , -2.2) node[draw,scale=0.2,diamond,line width=0.075mm]{}; 
	\draw (-1.16, -2.2) node[draw,scale=0.01,star,star point ratio=5, fill = black]{}; 
	\draw (-0.72 , -2.2) node[draw,scale=0.2,circle,line width=0.075mm]{}; 
	\draw (-0.57 , -2.2) node[draw,scale=0.2,diamond,line width=0.075mm]{}; 
	
	\end{tikzpicture}
	}
	\caption{Box plots of (a) relative mean values ($\mu^r$), relative standard deviation ($\sigma^r$) and (b) t-values for PIANO feature maps and ISLES 2017 maps, computed from 43 patients. $\star,\, \diamond,\, \circ$ indicate statistically significant differences between the PIANO feature maps and CBF, CBV, ADC respectively, based on a paired t-test with Bonferroni correction at a significance level of $0.05$. (Negative t-values indicate a metric's mean in the lesion is lower than the c-lesion. Lower is better.)}
	\label{box_plots}
\end{figure}


==> sub/exp_results/table_tmi.tex <==
\begin{table}[t]
\caption{Quantitative comparison between PIANO feature maps and ISLES 2017 maps over 43 subjects, using \emph{Mean}, \emph{Median}, \emph{Standard Deviation (STD)} of relative mean $\mu^r$, relative STD $\sigma^r$ (the lower the better), and t-value (higher absolute value indicates greater difference).} 
\resizebox{\linewidth}{!}{
\centering
    \begin{tabular}{P{1.2cm}P{1.2cm}P{1.2cm}P{1.2cm}P{1.2cm}P{1.2cm}P{1.2cm}P{1.2cm}P{1.2cm}P{1.2cm}} 
       \toprule \\[-4ex] 
       \multirow{2}{*}{ \thead{\\[-3ex]\normalsize\bf ~Maps~~~~}} &
  \multicolumn{3}{c}{\thead{\normalsize\bf  ~~ Relative Mean ($\mu^r$)~~}} &
  \multicolumn{3}{c}{\thead{\bf \normalsize ~~Relative STD ($\sigma^r$)~~}} &
  \multicolumn{3}{c}{\thead{\bf \normalsize ~~t-value~~}}  \\  [-1.4ex] 
   
     \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \\[-3.25ex] 
     &{ \normalsize \emph{Mean}} &{\normalsize{\emph{Median}}} & {\normalsize{\emph{STD}}} & {\normalsize \emph{Mean}} &{\normalsize{\emph{Median}}} & {\normalsize \emph{STD}} & { \normalsize \emph{Mean}} & {\normalsize{\emph{Median}}} & {\normalsize \emph{STD}} \\ [-0.4ex]
     \midrule\\[-2.75ex]
${\| {\bf{V}} \|_2}$ & {\bf 0.55} & {\bf 0.52} & {\bf 0.13} & 0.72 & 0.68 & 0.19 & {\bf -57.76} & {\bf -47.13}& {\bf 51.83} \\ [0.5ex]
$D$ & 0.60 & 0.56 & 0.19 & {\bf 0.56} & {\bf 0.56} & {\bf 0.18} & -29.51 & -20.58 & 27.67 \\ 
\midrule[0.1pt]\\[-2.75ex]
CBF & 0.57 & 0.55 & 0.19 & 0.66 & 0.61 & 0.23 & -32.43 & -26.08 & 27.68 \\[0.5ex]
CBV & 0.89 & 0.80 & 0.36 & 0.93 & 0.87 & 0.33 & -9.22 & -4.64 & 17.32  \\[0.5ex]
ADC & 0.76 & 0.78 & 0.14 & 0.80 & 0.82 & 0.27 & -20.46 & -13.50 & 19.63 \\[0.25ex]
          \bottomrule
    \end{tabular}
    \label{table}
}
\end{table}

==> sub/exp_results/table_tmi2_3maps.tex <==
\begin{table}[t]
\caption{Quantitative comparison between PIANO feature maps and ISLES 2017 maps over 43 subjects, using \emph{Mean}, \emph{Median}, \emph{Standard Deviation (STD)} of relative mean $\mu^r$, relative STD $\sigma^r$ (the lower the better), and t-value (higher absolute value indicates greater difference).} 
\resizebox{\linewidth}{!}{
\centering
    \begin{tabular}{P{0.5cm}P{1.5cm}P{1.2cm}P{1.2cm}P{1.2cm}P{1.2cm}P{1.2cm}} 
       \toprule \\[-2ex]
        \multicolumn{2}{c}{\bf Maps} & ${\| {\bf{V}} \|_2}$ & $D$ & CBF & CBV & ADC \\ [0.5ex]
     \midrule\\[-2ex]
       \parbox[t]{5mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\thead{Relative\\Mean ($\mu^r$)}}}} & {\emph{Mean}} & {\bf{0.55}}  & 0.60 & 0.57 & 0.89 & 0.76  \\ [1ex]
       &  {\emph{Median}} & {\bf{0.52}}  & 0.56 & 0.55 & 0.80 & 0.78 \\ [1ex]
       &  {\emph{STD}} & {\bf{0.13}}  & 0.19 & 0.19 & 0.36 & 0.14 \\ [0.75ex]
     \midrule\\[-2ex]
       \parbox[t]{5mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\thead{Relative\\STD ($\sigma^r$)}}}}  & {\emph{Mean}} & 0.72 & {\bf{0.56}} & 0.66 & 0.93 & 0.80  \\ [1ex]
       &  {\emph{Median}} & 0.68 & {\bf{0.56}} & 0.61 & 0.87 & 0.82 \\ [1ex]
       &  {\emph{STD}} & 0.19 & {\bf{0.18}} & 0.23 & 0.33 & 0.27 \\ [0.75ex]
     \midrule\\[-2ex]
       \parbox[t]{-6mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\thead{\bf{t-value~~~}}}}} & {\emph{Mean}} & {\bf{-57.76}}  & -29.51 & -32.43 & -9.22 & -20.46   \\ [1ex]
       &  {\emph{Median}} & {\bf{-47.13}}  & -20.58 & -26.08 & -4.64 & -13.50 \\ [1ex]
       &  {\emph{STD}} & {\bf{51.83}}  & 27.67 & 27.68 & 17.32 & 19.63 \\ [0.75ex] % [2ex]
          \bottomrule
    \end{tabular}
    \label{table}
}
\end{table}

==> sub/exp_results/table_tmi2_6maps.tex <==
\begin{table}[t]
\caption{Quantitative comparison between PIANO feature maps and ISLES 2017 maps over 43 subjects, using \emph{Mean}, \emph{Median}, \emph{Standard Deviation (STD)} of relative mean $\mu^r$, relative STD $\sigma^r$ (the lower the better), and absolute t-value (higher absolute value indicates greater difference).} 
\resizebox{\linewidth}{!}{
\centering
    \begin{tabular}{P{0.6cm}P{1.4cm}|P{0.65cm}P{0.65cm}|P{0.65cm}P{0.65cm}P{0.65cm}P{0.65cm}P{0.65cm}P{0.65cm}} 
       \toprule \\[-2ex]
        \multicolumn{2}{c|}{\bf Maps} & ${\| {\bf{V}} \|_2}$ & $D$ & ADC & CBF & CBV & MTT & TTP &Tmax \\ [0.5ex]
     \midrule\\[-2ex]
       \parbox[t]{5mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\thead{Relative\\Mean ($\mu^r$)}}}} & {\emph{Mean}} & {\bf{0.55}}  & 0.60 & 0.76 & 0.57 & 0.89 & 1.83 & 1.47 & 7.41  \\ [1ex]
       &  {\emph{Median}} & {\bf{0.52}}  & 0.56 & 0.78 & 0.55 & 0.80 & 1.59 & 1.46 & 6.77 \\ [1ex]
       &  {\emph{STD}} & {\bf{0.13}}  & 0.19 & 0.14 & 0.19 & 0.36 & 0.75 & 0.23 & 4.19 \\ [0.75ex]
     \midrule\\[-2ex]
       \parbox[t]{5mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\thead{Relative\\STD ($\sigma^r$)}}}}  & {\emph{Mean}} & 0.72 & {\bf{0.56}} & 0.80 & 0.66 & 0.93 & 2.09 & 2.40 & 5.42  \\ [1ex]
       &  {\emph{Median}} & 0.68 & {\bf{0.56}} & 0.82 & 0.61 & 0.87 & 1.80 & 1.85 & 3.51 \\ [1ex]
       &  {\emph{STD}} & 0.19 & {\bf{0.18}} & 0.27 & 0.23 & 0.33 & 0.97 & 2.01 & 5.22 \\ [0.75ex]
     \midrule\\[-2ex]
       \parbox[t]{5mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\thead{Absolute~~\\t-value~~}}}} & {\emph{Mean}} & {\bf{57.76}}  & 29.51 & 20.55 & 32.61 & 13.53 & 33.56 & 44.59 & 60.07  \\ [1ex]
       &  {\emph{Median}} & {\bf{47.13}}  & 20.58 & 13.50 & 26.08 & 8.48 & 18.52 & 28.87 & 46.49 \\ [1ex]
       &  {\emph{STD}} & {\bf{51.83}}  & 27.67 & 19.53 & 27.47 & 14.21 & 31.70 & 44.16 & 50.34  \\ [0.75ex] % [2ex]
          \bottomrule
    \end{tabular}
    \label{table}
}
\end{table}
